Shortest Paths in a Hybrid Network Model

We introduce a communication model for hybrid networks, where nodes have access to two different communication modes: a local mode where communication is only possible between specific pairs of nodes, and a global mode where communication between any pair of nodes is possible. This can be motivated, for instance, by wireless networks in which we combine direct device-to-device communication (e.g., using WiFi) with communication via a shared infrastructure (like base stations, the cellular network, or satellites). Typically, communication over short-range connections is cheaper and can be done at a much higher rate. Hence, we are focusing here on the LOCAL model (in which the nodes can exchange an unbounded amount of information in each round) for the local connections while for the global communication we assume the so-called node-capacitated clique model, where in each round every node can exchange only $O(\log n)$-bit messages with just $O(\log n)$ other nodes. In order to explore the power of combining local and global communication, we study the impact of hybrid communication on the complexity of computing shortest paths in the graph given by the local connections. Specifically, for the all-pairs shortest paths problem (APSP), we show that an exact solution can be computed in time $\tilde O\big(n^{2/3}\big)$ and that approximate solutions can be computed in time $\tilde \Theta\big(\!\sqrt{n}\big)$. For the single-source shortest paths problem (SSSP), we show that an exact solution can be computed in time $\tilde O\big(\!\sqrt{\mathsf{SPD}}\big)$, where $\mathsf{SPD}$ denotes the shortest path diameter. We further show that a $\big(1\!+\!o(1)\big)$-approximate solution can be computed in time $\tilde O\big(n^{1/3}\big)$. Additionally, we show that for every constant $\varepsilon>0$, it is possible to compute an $O(1)$-approximate solution in time $\tilde O(n^\varepsilon)$.

==> sections/lower_bounds.tex <==
% !TEX root = ../main.tex
\subsection{Lower Bounds for APSP}
\label{sec:lowerbounds}

%In this section we assume a slightly more general communication model
%and we allow that each node may send and receive up to $\sigma$ and
%$\rho$ $B=\Omega(\log n)$-bit messages, respectively, via global
%links. Note that the given lower bounds hold even if we do not assume
%that $B, \sigma, \rho \in \Theta(\log n)$.
%% In fact, non-trivial results are obtained for $\sigma \in o(k)$,
%% $\rho \in o(\ell)$ for token dissemination, and for
%% $\sigma \in \bigO(n^\varepsilon)$ with $\varepsilon < 1/2$ for APSP.
%% (Recall that $k$ is the total number of tokens and $\ell$ is the
%% maximum number of tokens that any node can begin with).
%We start by proving a technical lemma, which will afterwards be used
%in all the subsequent lower bounds.
%\fabian{Maybe, we should just assume that $B, \sigma, \rho = O(\log n)$
%and possibly add a remark at the end. One could add a similar lemma
%that allows to prove a linear in $\ell$ lower bound for token
%dissemination. I am not sure whether we want to add this for the
%submission to PODC. I would somehow keep the paper as focused as
%possible on the shortest path problems.}

In order to obtain rigorous lower bounds we introduce a technical lemma. It shows that for a class of graphs and a dedicated node $b$, we can create a bottleneck for the information that can be transmitted from parts of the graph to $b$ (c.f.\ Figure \ref{fig:lowerBounds}, left). Subsequently we show that obtaining solutions (or even approximations) for the all pair shortest path problem requires that a certain amount of information (measured in terms of its entropy) must be transmitted to $b$, which demonstrates the lower bounds claimed in this section.

%\phil{I don't know if we can afford pictures. Personally, as a reader I'm always grateful if I can see depiction of a construction that is made in a proof, so I would like to put it here, even though it consumes a lot of space.}

\begin{figure}[H]
	\centering
	\begin{subfigure}{.455\textwidth}
		\vspace*{4pt}
		\centering
		\includegraphics[width=0.92\linewidth]{img/lower_bound_APSP_lemma_compressed.pdf}
		%\caption{Depiction of the Lemma \ref{lem:lowerboundlemma}.}
		\label{fig:lowerBoundAPSPapproxlemma}
	\end{subfigure}%
	\begin{subfigure}{.54\textwidth}
		\vspace*{4pt}
		\centering
		\includegraphics[width=0.92\linewidth]{img/lower_bound_APSP_approx_compressed.pdf}
		%\caption{Depiction of the Theorem \ref{thm:lowerBoundAPSPapprox}.}
		\label{fig:lowerBoundAPSPapprox}
	\end{subfigure}
	\caption{Construction of Lemma \ref{lem:lowerboundlemma} (left) and of Theorem \ref{thm:lowerBoundAPSPapprox} (right).}
%	\label{fig:test}
	\label{fig:lowerBounds}
\end{figure}

%\begin{figure}[H]
%	\centering
%	\includegraphics[width=0.55\linewidth]{img/lower_bound_APSP_lemma.pdf}
%	\caption{Depiction of the Lemma \ref{lem:lowerboundlemma}.}
%	\label{fig:lowerBoundAPSPapproxlemma}
%\end{figure}



We use Lemma \ref{lem:lowerboundlemma} to show a lower bound of \smash{${\Omega}\big(\!\sqrt{n}/\log n\big)$} for APSP that is robust even if we allow approximation factors up to $\bigO\big(\!\sqrt{n} \!\cdot\! \log n\big)$.

%Finally, we show a lower bound that differs from the one above only by a \smash{$1/\sqrt{\log n}$} factor, but is robust even if we allow approximation factors up to $\bigO\big(\!\sqrt{n} \!\cdot\! \log n\big)$. The idea is to construct an unweighted graph consisting of a path of length $\Omega(n)$ and two node sets $S_1,S_2$ of size $\Omega(n)$ each. Let $b$ be the first node on the path. Then we attach $S_1$ and $S_2$ to nodes on the path at distance approximately $\Omega(\!\sqrt{n})$ and $\Omega(n)$ from $b$, respectively (c.f.\ Figure \ref{fig:lowerBoundAPSPapprox}). 
%
%Now assume an adversary ``shuffles'' the nodes in $S_1,S_2$ uniformly at random. If $b$ does not know for a node $u$ whether $u \in S_1$ or $u \in S_2$, then $b$ must assume $u \in S_2$ (recall that approximations must be lower bounded by the true distance). However, if $u \in S_1$ is true, then this results in a larger approximation ratio than what we allow. In order to learn the distances to \textit{all} nodes in $S_1,S_2$ the node $b$ needs to learn at least which nodes are in $S_1$. We show that this requires that $b$ needs to receive $\Omega(n)$ bits.

\begin{theorem}
	\label{thm:lowerBoundAPSPapprox}	
	An \smash{$\alpha$}-approximative APSP algorithm in the hybrid network model on unweighted graphs takes \smash{${\Omega}\big(\!\sqrt{n}/\log n\big)$} rounds, for any $\alpha \leq {\sqrt{nc}\cdot\log n}/{2}$, where $c \log n$ (for constant $c > 0$) is the number of messages a node can receive per round over global edges.
\end{theorem}

\begin{proof}[Proof Sketch]
 The idea is to construct an unweighted graph consisting of a path of length $\Omega(n)$ and two node sets $S_1,S_2$ of size $\Omega(n)$ each. Let $b$ be on one end of the path. Then we attach nodes sets $S_1$ and $S_2$ of size $\Omega(n)$ to the path at distance approximately $L \in \tilOm(\!\sqrt{n})$ and $\Omega(n)$ from $b$ (c.f.\ Figure \ref{fig:lowerBounds}, right). 
	
	Now assume an adversary ``shuffles'' the nodes in $S_1,S_2$ uniformly at random, where the state of $S_1$ will be our random variable $X$. If $b$ does not know for a node $u$ whether $u \!\in\! S_1$ or $u \!\in\! S_2$, then $b$ must assume $u \in S_2$ (recall that approximations must be lower bounded by the true distance). However, if $u \in S_1$ is true, then this results in a larger approximation ratio than we allow. We show that in order to learn $S_1$, node $b$ needs to receive $H(X)=\Omega(n)$ bits. Choosing $L \in \Theta(\sqrt{n}/\log n)$ yields the claimed lower bound.
\end{proof}

%\begin{figure}[H]
%	\vspace*{-0.3cm}
%	\centering
%	\includegraphics[width=0.58\linewidth]{img/lower_bound_APSP_approx.pdf}
%	\caption{Node $b$ must receive $\Omega(n)$ bits to learn $S_1$, $S_2$.}
%	\label{fig:lowerBoundAPSPapprox}
%\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/model.tex <==
\subsection{Preliminaries and Problem Definitions}


%\phil{I think we need a discussion about nomenclature to agree on one common standard which we use throughout the whole paper. I started a list further below to see what kind of formulations are in use right now and to have a starting point for a discussion (feel free to add to list). I (tentatively) reintroduced the clique $G' = \big(V, \binom{n}{2} \big)$ (I think you call it logical graph) because for brevity I tend to use $G'$ a lot instead of logical graph (but it can be changed if we settle on not using $G'$). Moreover I (tentatively) reintroducced the terms $\sigma$ and $\rho$ for the send/receive restrictions of node, because the lower bounds give meaningful results also for values other than $\Theta(\log n)$ (I wrote a small note in the beginning of the section on lower bounds).}
%
%{\begin{table*}[h]
%	\centering
%	\begin{tabular}{@{}p{0.25\textwidth} p{0.3\textwidth} p{0.4\textwidth}}
%		\toprule
%			expression & meaning & notes \\
%		\midrule
%		\midrule
%			$G'$ & clique formed by ``long range/ logical links'' & I prefer to keep things brief, and use abbreviations where possible\\				
%		\midrule
%			physical/locigal edges & edges of $G$ and $G'$ &  \\
%		\midrule
%			``send a message via $G'$'' & send a message via a long range link/ logical edge & since we have to say this a lot it in my opinion makes sense to keep it as short as possible. This is what I came up with and used so far.\\
%		\midrule
%			HYBRID or HYBRID-LOCAL model& suggestions for the model name & in the tradition of using all caps for model names\\
%		\bottomrule
%	\end{tabular}
%	\caption{(Tentative) nomenclature nd naming suggestions for the paper.}
%\end{table*}}

The \emph{distance} between any two nodes $u,v \in V$ of a graph $G$ is defined as 
\[
    d_G(u,v) := \!\!\min_{\text{$u$-$v$-path } P}\, w(P),
\]
where $w(P) = \sum_{e \in P}w(e)$ denotes the length of a path $P$.
A path between two nodes with smallest length is called a \emph{shortest path}.
The \emph{hop-distance} between two nodes $u$ and $v$ is defined as
\[
    hop_G(u,v) := \min_{\text{$u$-$v$-path } P} |P|,
\]
where $|P|$ denotes the number of edges (or \emph{hops}) of a path $P$.
Let the \emph{$h$-limited distance} from $u$ to $v$:
\[ 
    d_{h,G}(u,v) := \!\!\min_{\substack{\text{$u$-$v$-path } P\\ |P| \leq h }}\, w(P).
\]
If there is no $u$-$v$ path $P$ with $|P|\leq h$, then $d_{h,G}(u,v) := \infty$. The \emph{diameter} $D(G)$ of $G$ is defined as the length of any shortest path in $G$, and the \emph{shortest-path diameter} $\SPD(G)$ is the minimum number such that $d_{\SPD(G),G}(u,v)=d_G(u,v)$ for all $u,v\in V$. 
Whenever the graph $G$ is clear from the context, we drop the subscript $G$ in the above notations. %, i.e., we use $d(u,v)$, $hop(u,v)$, and $d_h(u,v)$ instead of $d_G(u,v)$, $hop_G(u,v)$, and $d_{h,G}(u,v)$.
In this paper, we consider the following shortest-paths problems in $G$.

\vspace*{-4mm}

\paragraph{All-Pairs Shortest Paths Problem (APSP).} Every node $u \in V$ has to learn $d(u,v)$ for all $v \in V$. In the $\alpha$-approximate APSP problem for some $\alpha>1$, every node $u\in V$ has to learn values $d'(u,v)$ such that $d(u,v)\leq d'(u,v)\leq \alpha\cdot d(u,v)$ for all $v\in V$.

\vspace*{-4mm}

\paragraph{Single-Source Shortest Paths Problem (SSSP).} There is a source $s \in V$ and every node $u \in V$ has to learn $d(u,s)$. In the $\alpha$-approximate SSSP problem for some $\alpha>1$, every node $u\in V$ has to learn $d'(u,s)$ such that $d(u,s)\leq d'(u,s)\leq \alpha\cdot d(u,s)$.

\medskip

In order to solve shortest path problems efficiently, we also show how to solve the \textit{$(k,\ell)$-token dissemination problem ($(k,\ell)$-TD)}. Here we are given a set of $k$ tokens each of size $O(\log n)$-bits that need to be learned by all nodes $v\in V$. Initially, each token is known by one node and no node initially possesses more than $\ell$ tokens.

As a byproduct of our exact SSSP algorithm, we solve the \textit{$h$-limited $k$-source shortest paths problem ($(h,k)$-SSP)}, in which there is a set $S \subseteq V$ of $k$ sources and a parameter $h \ge 1$ and every node $u \in V$ has to learn $d_h(u,s)$ for every $s \in S$. 





